Level-S$^2$fM: Structure from Motion on Neural Level Set of Implicit Surfaces

This paper presents a neural incremental Structure-from-Motion (SfM) approach, Level-S$^2$fM, which estimates the camera poses and scene geometry from a set of uncalibrated images by learning coordinate MLPs for the implicit surfaces and the radiance fields from the established keypoint correspondences. Our novel formulation poses some new challenges due to inevitable two-view and few-view configurations in the incremental SfM pipeline, which complicates the optimization of coordinate MLPs for volumetric neural rendering with unknown camera poses. Nevertheless, we demonstrate that the strong inductive basis conveying in the 2D correspondences is promising to tackle those challenges by exploiting the relationship between the ray sampling schemes. Based on this, we revisit the pipeline of incremental SfM and renew the key components, including two-view geometry initialization, the camera poses registration, the 3D points triangulation, and Bundle Adjustment, with a fresh perspective based on neural implicit surfaces. By unifying the scene geometry in small MLP networks through coordinate MLPs, our Level-S$^2$fM treats the zero-level set of the implicit surface as an informative top-down regularization to manage the reconstructed 3D points, reject the outliers in correspondences via querying SDF, and refine the estimated geometries by NBA (Neural BA). Not only does our Level-S$^2$fM lead to promising results on camera pose estimation and scene geometry reconstruction, but it also shows a promising way for neural implicit rendering without knowing camera extrinsic beforehand.

==> docs/algorithm.tex <==
% \begin{document}
% 	\begin{algorithm}	
% 		\caption{Thank you my darling}\label{algorithm}
% 		\KwIn{\\
% 			The point \bm{$x$}\;
% 			The good thing \bm{${x_a}$}\;
% 			The label \bm{$y$}\;	
% 			}			
% 		\KwOut{\\The prediction \bm{${L_{pred}}$}\;}		
% 		\textbf{Initialization}:\\			
% 		\tcc{Calculate the loss by using the adversarial loss function $adv\_loss\left( {{\rm{\cdot}},{\rm{\cdot}}} \right)$}		
% 		$loss \leftarrow adv\_loss\left( {f\left( {x_{adv}} \right),L} \right)$\;
% 		\For{$n \leftarrow 0$ \KwTo $N$}
% 			{
% 				$y \leftarrow {x_a}$\;
% 				\If{$x =  = {x_a}$}
% 					{$alright!$\;
% 					 $break;$
% 					}
% 			}											
% 	\end{algorithm}
% \end{document}
\begin{algorithm}	
    \caption{Closest Surface Tracking Bundle Adjustment}
    \label{algorithm}
    \KwIn{\\
        The point set \bm{$\mathcal{X}^{\text{in}}$}\;
        The signed distance function \bm{${sdf}$}\;
        The feature tracks \bm{$\mathcal{F}$}\;	
        The camera poses \bm{$\mathcal{P}$}\;
        The radiance filed \bm{$rad$}\;
        The ground truth images \bm{$\mathcal{I}$}\;
        }			
    \KwOut{\\
    The new point set \bm{$\mathcal{X}^{\text{out}}$}\;
    The optimized camera poses \bm{$\mathcal{P}^{\text{out}}$}\;
    The optimized signed distance function \bm{${sdf}^{\text{out}}$}\;
    The radiance filed \bm{${rad}^{\text{out}}$};\
    }		
    \textbf{Bundle Adjustment on Neural Level Sets}:\\			
    \tcc{Calculate the reprojection of using the function of $reproj\_loss(\mathcal{X}^{i},\mathcal{F},\mathcal{P})$;\\ 
    Calculate the rendering loss of using the $rend\_loss(\mathcal{P},{rad},\mathcal{I})$ function}	
    \For{$n \leftarrow 0$ \KwTo $N$}
        {
            \If{$n =  = 0$}
                {$\mathcal{X}^{0}=\mathcal{X}^{\text{in}}$\;
                $\mathcal{P}^{0}=\mathcal{P}$\;
                $sdf^{0}=sdf$\;
                $rad^{0}=rad$
                }
            $\mathcal{X}^{n}=\mathcal{X}^{n-1}-\nabla sdf(\mathcal{X}^{n})sdf(\mathcal{X}^{n}) $\;
            $\mathcal{L}_{\text{reproj}}^{\text{mask}}=reproj\_loss(\mathcal{X}^{n},\mathcal{F},\mathcal{P}^{n})$\;
            $\mathcal{L}_{\text{rend}}=rend\_loss(\mathcal{P}^{n},{rad}^{n},\mathcal{I})$\;

            $\mathcal{L}_{\text{total}}=\mathcal{L}_{\text{rend}}+\mathcal{L}_{\text{reproj}}^{\text{mask}}$\;
            backward\;
            $\mathcal{P}^{n} \rightarrow \mathcal{P}^{n+1}, sdf^{n} \rightarrow sdf^{n+1}, rad^{n} \rightarrow rad^{n+1}$;\
            
        }											
\end{algorithm}


% $loss \leftarrow adv\_loss\left( {f\left( {x_{adv}} \right),L} \right)$\;

==> figures/Experiment/experiment.tex <==
\begin{figure}[htbp]
% \centering
\includegraphics[width=.48\textwidth]{figs/expfig1.pdf}
\caption{\textbf{2D Mismatches and SDF rejection.} .}
\label{fig:exp1}
\end{figure}

==> figures/method/pipeline.tex <==
\begin{figure*}
\centering
%\scalebox{1.1}{
\includegraphics[width=.96\linewidth]{figs/pipeline_final.pdf}
% }
\caption{\textbf{Overview of Level-S$^{2}$fM.} We learn to do geometric calculations including Triangulation, PnP and Bundle Adjustment above neural level sets, which easily help to reject the outliers in the matches especially in the texture repeated scenes. Also, due to the continuous surface priors of neural level sets, we achieve better pose estimation accuracy and our reconstructed points are sticking on the surface which are painted with color in the figure. While, there are a lot of outlier 3d points reconstructed by COLMAP~\cite{COLMAP} which are painted by black.}
\label{fig:pipeline}
\end{figure*}
